Optimal Approximate Matrix Multiplication over Sliding Window

Matrix multiplication is a core operation in numerous applications, yet its exact computation becomes prohibitively expensive as data scales, especially in streaming environments where timeliness is critical. In many real-world scenarios, data arrives continuously, making it essential to focus on recent information via sliding windows. While existing approaches offer approximate solutions, they often suffer from suboptimal space complexities when extended to the sliding-window setting. In this work, we introduce SO-COD, a novel algorithm for approximate matrix multiplication (AMM) in the sliding-window streaming setting, where only the most recent data is retained for computation. Inspired by frequency estimation over sliding windows, our method tracks significant contributions, referred to as snapshots, from incoming data and efficiently updates them as the window advances. Given matrices \(\boldsymbol{X} \in \mathbb{R}^{d_x \times n}\) and \(\boldsymbol{Y} \in \mathbb{R}^{d_y \times n}\) for computing \(\boldsymbol{X} \boldsymbol{Y}^T\), we analyze two data settings. In the \emph{normalized} setting, where each column of the input matrices has a unit \(L_2\) norm, SO-COD achieves an optimal space complexity of \( O\left(\frac{d_x+d_y}{\epsilon}\right) \). In the \emph{unnormalized} setting, where the square of column norms vary within a bounded range \([1, R]\), we show that the space requirement is \( O\left(\frac{d_x+d_y}{\epsilon}\log R\right) \), which matches the theoretical lower bound for an \(\epsilon\)-approximation guarantee. Extensive experiments on synthetic and real-world datasets demonstrate that SO-COD effectively balances space cost and approximation error, making it a promising solution for large-scale, dynamic streaming matrix multiplication.

==> algorithms/alg-1-COD.tex <==
\begin{algorithm}[t]
    \caption{Co-Occurring Directions (COD)}
    \label{alg:cod}
    \DontPrintSemicolon
    \KwInput{$\boldsymbol{X}\in \mathbb{R}^{d_x\times n}$, $\boldsymbol{Y}\in \mathbb{R}^{d_y\times n}$ and sketch size $l$}
    \KwOutput{$\boldsymbol{A}\in \mathbb{R}^{d_x\times l}$ and $\boldsymbol{B}\in \mathbb{R}^{d_y\times l}$}

    Initialize $\boldsymbol{A} \leftarrow 0^{d_x\times l},\ \boldsymbol{B} \leftarrow 0^{d_y\times l}$\;
    
    \For{$i = 1 \sim n$}{
        Insert $\boldsymbol{x}_i$ into a zero valued column of $\boldsymbol{A}$
        
        Insert $\boldsymbol{y}_i$ into a zero valued column of $\boldsymbol{B}$
        
        \If{$\boldsymbol{A}$ or $\boldsymbol{B}$ has no zero valued columns}
        {
            $(\boldsymbol{Q}_x, \boldsymbol{R}_x) \leftarrow QR(\boldsymbol{A})$

            $(\boldsymbol{Q}_y, \boldsymbol{R}_y) \leftarrow QR(\boldsymbol{B})$

            $[\boldsymbol{U},\boldsymbol{\Sigma},\boldsymbol{V}] \leftarrow SVD(\boldsymbol{R}_x\boldsymbol{R}_y^T)$

            $\delta \leftarrow \sigma_{l/2}(\boldsymbol{\Sigma})$

            $\hat{\boldsymbol{\Sigma}} = max(\boldsymbol{\Sigma} - \delta \boldsymbol{I}_l, 0)$

            $\boldsymbol{A} \leftarrow \boldsymbol{Q}_x\boldsymbol{U}\sqrt{\hat{\boldsymbol{\Sigma}}}$
            
            $\boldsymbol{B} \leftarrow \boldsymbol{Q}_y\boldsymbol{V}\sqrt{\hat{\boldsymbol{\Sigma}}}$
        }
    }

    \Return $\boldsymbol{A},\boldsymbol{B}$
    
\end{algorithm}

==> tables/tab-1-notation.tex <==
\begin{table}[t]
  \caption{Frequently used notations.}
  \vspace{-4mm}
  \label{tab:table-notations}
  \begin{tabular}{|l|l|}
    \hline
    Notations & Descriptions\\
    \hline
    $\mathcal{G}=(\mathcal{V},\mathcal{E})$ & A graph with node set and edge set\\
    \hline
    $n,m$ & The number of nodes and edges\\
    \hline
    $c,F$ & The number of classes and features\\
    \hline
    $\mathcal{L},\mathcal{U}$ & The labelled set and unlabelled set\\
    \hline
    $\vect{A},\vect{D},\vect{X},\vect{\mathcal{Y}}$ & Adjacent, degree, feature, and label matrix\\
    \hline
    $\mathcal{N}(v)$ & The set of out-neighbors of node $v$\\
    \hline
    $\vect{Z}$ & The output matrix of GNN\\
    \hline
    $\mathcal{M},\mathcal{B}$ & The training model and labelling budget\\
    \hline
    $\alpha, \theta$ & The stopping probability and threshold of PPR\\
    \hline
    $d,\eta_d$ & Reachable parameter and threshold of diversity\\
    \hline
    $\vect{\pi}_u(v)$ & The PPR value of $v$ with respect to $u$\\
    \hline
    $\phi(u), \phi(S)$ & The set of nodes covered by node $u$ and set $S$\\
    \hline
\end{tabular}
\end{table}

==> tables/tab-2-data-sets.tex <==
\begin{table}[t]
  \caption{Dataset statistics.}
  \vspace{-4mm}
  \label{tab:table-data-sets}
  \begin{tabular}{lrrcc}
    \toprule
    Name & Nodes & Edges & Classes & Features \\
    \midrule
    Cora       &   2,708  &      5,429 &  7 & 1,433 \\
    Citeseer   &   3,327  &      4,732 &  6 & 3,703 \\
    Pubmed     &  19,717  &     44,338 &  3 &   500 \\
    Reddit     & 232,965  & 11,606,919 & 41 &   602 \\
     \bottomrule
\end{tabular}
\end{table}

